Enhancing Review Comprehension with Domain-Specific Commonsense

Review comprehension has played an increasingly important role in improving the quality of online services and products and commonsense knowledge can further enhance review comprehension. However, existing general-purpose commonsense knowledge bases lack sufficient coverage and precision to meaningfully improve the comprehension of domain-specific reviews. In this paper, we introduce xSense, an effective system for review comprehension using domain-specific commonsense knowledge bases (xSense KBs). We show that xSense KBs can be constructed inexpensively and present a knowledge distillation method that enables us to use xSense KBs along with BERT to boost the performance of various review comprehension tasks. We evaluate xSense over three review comprehension tasks: aspect extraction, aspect sentiment classification, and question answering. We find that xSense outperforms the state-of-the-art models for the first two tasks and improves the baseline BERT QA model significantly, demonstrating the usefulness of incorporating commonsense into review comprehension pipelines. To facilitate future research and applications, we publicly release three domain-specific knowledge bases and a domain-specific question answering benchmark along with this paper.

==> eval.tex <==
\subsection{Datasets}
\begin{itemize}
    \item Aspect-based sentiment analysis (ABSA) of 2000 data points (ready). The ABSA dataset contains 100 reviews about a hotel in Chicago. For each review, we target 14 common hotel aspects based on tags from www.booking.com. They are ``Location'', ``Staff'', ``Cleaniness'', ``Staff'', ``Price'', ``Spaciousness'', ``Quietness'', ``Bedding'', ``Parking'', ``Facilities'', ``Wifi'', ``Views'', ``Spa \& Gym''. To collect the dataset, we launched a crowd-sourcing task on Figure Eight, asking human annotators to highlight the positive and negative sentences about each aspect. We also (plan to) ask annotators to label the overall sentiment about each aspect.
    \item Question-answering with real yelp questions of 400 QA pairs. (by Sep 6th)
\end{itemize}

\subsection{Exp 1: HotelSense vs. other models on ABSA task.}
\label{exp:absa}
We compare the following models on ABSA task based on precision, recall and F1 score.
\begin{enumerate}
    \item ExtractRRC (our model) + HotelSense
    \item ExtractRRC + ConceptNet
    \item KBLSTM~\cite{Bishan2017} + HotelSense
    \item BERT~\cite{Jacob2019}
    \item Review-tuned BERT
    \item Explain-yourself approach: use the conclusion text instead of representation as input to the QA model.
\end{enumerate}

The hypotheses that we want to prove by these comparisons are as follows:

\begin{itemize}
    \item Domain-specific commonsense knowledge complements language models (by comparing 1,4,5)
    \item Domain-specific commonsense knowledge complements general commonsense knowledge bases (by comparing 1,2)
    \item The commonsense integration architecture is better than the state-of-the-art. (by comparing 1,3)
    \item Building a commonsense knowledge graph is more cost-effective than training a language model with more training data (by comparing 1,5 while increasing the volume of reviews used for fine-tuning.)
\end{itemize}

\subsection{Exp 2: HotelSense vs. other models on hotel QA.}
Most are the same as Section~\ref{exp:absa}. We replace 3 with Review reading comprehension model (RRC model) from ~\cite{Hu2019}.

We also want to evaluate the performance of our commonsense model. We want to know (1) how many generated conclusions are correct commonsense, (2) how many of them are non-trivial commonsense?


% \begin{table}[t]
% \small
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     Model & Precision & Recall & F1 score \\ \hline
%     SOTA ABSA (which one?) & ?? & ?? & ??\\ \hline
%     SOTA ABSA with commonsense & ?? & ?? & ??\\ \hline 
%     \end{tabular}
%     \caption{Comparison between using state-of-the-art ABSA tool with and without commonsense.}
%     \label{tab:para_exp}
% \end{table}




% \subsection{Comparison with BERT}
% We want to show that the commonsense we collected is not captured by BERT.

% \subsection{Comparison with ConceptNet}
% We intend to show that a general-purpose commonsense knowledge base cannot help review comprehension tasks as much as our domain-specific commonsense knowledge base.

% \subsection{Comparison between our multi-task approach with KBLSTM}
% Existing baselines look up corresponding knowledge for tokens in the knowledge base. This works for a general-purpose commonsense knowledge base, but not for a domain-specific knowledge base. Generalization is an important property for integrating domain-specific commonsense into downstream tasks. The comparison between our solution and KBLSTM prove this.

% \begin{table}[t]
% \small
%     \centering
%     \begin{tabular}{|c|c|c|}
%     \hline
%     Model & Exact match & F1 score \\ \hline
%     ExtractRRC & 26.9\% & 46.0\%\\ \hline
%     KBLSTM & ?? & ??\\ \hline 
%     \end{tabular}
%     \caption{Comparison between ExtractRRC (our model) and KBLSTM on the 200 QA dataset.}
%     \label{tab:para_exp}
% \end{table}

% We hope the evaluation can provide evidence for the following hypotheses: (1) Commonsense improves review comprehension tasks, such as aspect-based sentiment analysis and question answering, (2) domain-specific commonsense complements general commonsense knowledge bases. (3) building a knowledge graph is preferable compared to providing more training data, especially when the training data is relatively small. (4) The knowledge distillation method we develop is suitable for domain-specific commonsense knowledge bases and outperforms baseline integration methods.

==> impl.tex <==
\newcommand{\attr}{\ensuremath{\mathsf{attr}}}
\newcommand{\asp}{\ensuremath{\mathsf{as}}}
\newcommand{\opi}{\ensuremath{\mathsf{op}}}
\newcommand{\opinedb}{\ensuremath{\mathsf{OpineDB}}}


We implement our system in PyTorch. This section can be omitted if there is not much to write about.

\yuliang{added the following}
The implementation of \systemname\ leverages the \opinedb\ opinion extractor to extract
opinions from review text. Specifically, the extractor takes a single review 
(e.g., ``The bathroom is very clean but the food is average at best.'')
as input and outputs a set of tuples of form $(\attr, \opi, \asp)$ where 
$\attr$ is the category of the opinion (e.g., \textbf{Cleanliness}),
$\opi$ is the opinion modifier (e.g., ``very clean'') and
$\asp$ is the opinion aspect (e.g., ``bathroom'').

The extractor consists of 3 models, \emph{tagging}, \emph{pairing}, and attribute
\emph{classification} illustrated in Figure \ref{fig:opinedb}.
The tagging model identifies all spans of $\asp$ and $\opi$ via sequence tagging.
The pairing model checks whether each $(\opi, \asp)$ candidate pair is correct or not.
Next, the attribute classifier assigns each correct pair to a category opinions.
All 3 models are based on BERT and fine-tuned with training data that we obtained from
\cite{opinedb}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/xSense_extractor.pdf}
    \caption{The opinion extractor.}
    \label{fig:opinedb}
\end{figure}


==> system.tex <==
\subsection{Collection of commonsense}
% We introduce two ways of collecting domain-specific commonsense. (1) Free-text crowd-sourcing, (2) Universal schema on review extractions.
\begin{itemize}
    \item Free-text crowd-sourcing
    \item Universal schema on review extractions
\end{itemize}

\subsection{Representation of commonsense}
\begin{itemize}
    \item We identify three types of domain-specific commonsense: (1) inferences, (2) paraphrases, (3) ontology relationships.
    \item We build a knowledge graph to represent and maintain commonsense. The size of the knowledge graph is expected to have 5,000 nodes, and 7,500 edges.
\end{itemize}

\subsection{Integration of commonsense in language models}
% We develop an architecture that distills commonsense knowledge into BERT by co-training BERT with an auxiliary task that predicts commonsense. We introduce the following components in detail.
\begin{itemize}
    \item Our domain-specific knowledge base is not large-scale. This causes problems for search-based existing works. We develop a new model to apply domain-specific knowledge base with generalization. 
    \item An auxiliary commonsense language model that predicts conclusions for a given premise. (why do we choose a language model encoding commonsense? A small-sized knowledge graph needs generalization. How to make sure that the commonsense knowledge we found are representative.)
    \item Distilling commonsense knowledge by co-training the auxiliary model with BERT.
\end{itemize}
